The Cluster Lensing and Supernova Survey with Hubble (CLASH): Strong Lensing Analysis of Abell 383 from 16-Band HST WFC3/ACS Imaging

We examine the inner mass distribution of the relaxed galaxy cluster Abell 383 in deep 16-band HST/ACS+WFC3 imaging taken as part of the CLASH multi-cycle treasury program. Our program is designed to study the dark matter distribution in 25 massive clusters, and balances depth with a wide wavelength coverage to better identify lensed systems and generate precise photometric redshifts. This information together with the predictive strength of our strong-lensing analysis method identifies 13 new multiply-lensed images and candidates, so that a total of 27 multiple-images of 9 systems are used to tightly constrain the inner mass profile, $d\log \Sigma/d\log r\simeq -0.6\pm 0.1$ (r<160 kpc). We find consistency with the standard distance-redshift relation for the full range spanned by the lensed images, 1.01<z<6.03, with the higher redshift sources deflected through larger angles as expected. The inner mass profile derived here is consistent with the results of our independent weak-lensing analysis of wide-field Subaru images, with good agreement in the region of overlap. The overall mass profile is well fitted by an NFW profile with M_{vir}=(5.37^{+0.70}_{-0.63}\pm 0.26) x 10^{14}M_{\odot}/h and a relatively high concentration, c_{vir}=8.77^{+0.44}_{-0.42}\pm 0.23, which lies above the standard c-M relation similar to other well-studied clusters. The critical radius of Abell 383 is modest by the standards of other lensing clusters, r_{E}\simeq16\pm2\arcsec (for z_s=2.55), so the relatively large number of lensed images uncovered here with precise photometric redshifts validates our imaging strategy for the CLASH survey. In total we aim to provide similarly high-quality lensing data for 25 clusters, 20 of which are X-ray selected relaxed clusters, enabling a precise determination of the representative mass profile free from lensing bias. (ABRIDGED)

==> RefRepSec1.tex <==
Dear Editor,
we deeply thank the referee again for valuable comments. We detail in turn below the corresponding changes made.
Thank you,
The CLASH team.


Reviewer's Comments:
\emph{I thank the authors for their revision of the manuscript and answers to my comments. I have still a few comments on the revised version, more specifically one major comment (#1) and a few more minor revisions. I detail my comments below.}

Comment1:
%%-how are the cluster galaxies modelled in the analysis ? Which %% galaxies have been chosen for this purpose ? If this
%% improves the detection and photometry of lensed objects,this
%% would be useful to provide a separate
%% panel Fig. 3 showing the same image once the cluster galaxies
%% have been modelled and subtracted.

%In fact, we did not use the subtracted images for the %photometry (and redshift estimates)

\emph{I simply disagree with this approach. In the first version I did not comment because I implicitly thought that the light of all the bright elliptical galaxies in the cluster had been modelled and subtracted before any photometry on the multiple images is done. The way the photometry is done, including all this contaminating light, will bias any kind of photometric redshift depending on the location of the multiple images compared to bright cluster members, especially the BCG. As a minimal revision, I ask the authors to model and subtract the BCG in order to check their multiple imaged systems (such as system 8) which do not show a perfect agreement in their photo-z.}

We have now clarified this in the text, and indeed added a panel to Figure 3 showing a BCG-subtracted image. For the photometry we did model and subtract cluster galaxies but found that this did not yield significant photo-z improvements for most of our multiply lensed galaxies.  Galaxy modeling and subtracting should yield superior results, though highly robust and consistent modeling is required to yield quality 16-band photometry. Toward this end, we are currently developing a new and very promising technique.  In response to the referee's request, we have redone our galaxy modeling this time subtracting only the BCG, but significant photo-z improvements were not found.

We note the referee cited disagreement in the two halves of the arc denoted system 8.  In fact the two agree formally within the large error bars.  This arc suffers from from a common photo-z degeneracy (between z ~ 0.3 and ~3.0) which is difficult to break given the large photometric uncertainties of this low surface brightness object.  Agreement was not improved by modeling and subtracting the BCG and/or other cluster galaxies.

We also note that the few discrepant photo-z's are generally isolated to one image or so within each system which is an obvious counter-image but is fainter and/or more contaminated by cluster light.  The other images within each system provide more confident and reliable photo-z's.  Thus we believe our photo-z's for each system (each lensed galaxy) are secure as inputs to our mass model. Discrepant photo-z's for individual images therefore have no effect on the mass model, since we adopt for each system the most probable redshift as implied by the majority of images in that system, excluding the outliers. In cases of ambiguity the mass model itself can also aid us to determine which redshift is preferable, since although it may not be primarily calibrated to the right redshifts (or lensing distance ratios), it is primarily physical enough to at least imply which out of any given systems is at a higher redshift, thus helping is breaking possible degeneracies. In future work, we will continue to work toward more robust photo-z's for every lensed image, also in the context of member galaxies subtraction.

To make these clearer in the text, after the following sentence: ``The distances to the galaxies are, of course, key ingredients to the lens model.
The photo-z analyses used here also clearly aid us in assessing the robustness of the multiple-image identifications.'' , we added -->

``The photometry of some lensed images may be significantly contaminated by brighter nearby cluster galaxies.  SExtractor attempts to correct for this by measuring and subtracting the local background around each object.  This works well in some cases but not all.  To better reveal these lensed galaxies, we have carefully modeled and subtracted the light of several cluster galaxies including the BCG.  While this improved the detection of some lensed galaxies, it did not consistently improve their photometry and thus photometric redshifts.  The cluster galaxy wings must be modeled and subtracted very robustly and consistently to achieve quality photometry in all 16 bands for faint, nearby galaxy images.

Explicitly, for its subtraction, the BCG has been modeled using the CHEF basis \citep{Jiemenez&Benitez2011}. This
basis comprises both Chebyshev rational and trigonometric functions,
ensuring that the extended disk of this object is properly modeled. The
flexibility of the CHEFs scale parameter allows us to accurately represent
the BCG while keeping significant substructure and
arcs unchanged. An example of the BCG subtraction is seen in Figure \ref{curves383}. ''


Comment 2
%%-Somewhat related to the previous comment, the "BPZ analysis"
%% is supplemented by the "LPZ method". How does that work ? At
%% least a sentence summarizing the purpose of each method would
%% be useful.
%We have now changed the text:
%Based on the 16-filters photometry, we obtain photometric %redshifts using BPZ \citep{Benitez2000, Benitez2004, Coe2006}. %In addition, in order to cross-check our results,
%we derive the photometric redshifts for the arcs also using %LePhare (LPZ hereafter). These photometric redshifts are based %on a template fitting procedure with a $\chi^{2}$ estimation, %where we use the SED library developed for the COSMOS survey %\citep{Koekemoer2007}. The templates in use are synthetic
% spectra from \citet{BC03}, which are then calibrated
%using the spectroscopic redshifts available in the COSMOS area %as described in \citet{Ilbert2009}.
%to -->
%Based on the 16-filter photometry,
%we obtain photometric redshifts using BPZ \citep{Benitez2000,
%Benitez2004, Coe2006}
%and LePhare (LPZ hereafter; %\citealt{ArnoutsLPZ1999,Ilbert2006BPZ}).
%These two methods yielded some of the best results
%of all photo-z methods tested by the PHoto-z Accuracy Testing %group
%\citep{Hildebrandt2010PHOTZ}.
%BPZ and LPZ are similar in that spectral energy distribution %(SED)
%templates
%are basically redshifted and fit to observed photometry.
%BPZ currently uses 6 templates from PEGASE %\citep{Fioc1997PEGASE},
%calibrated using the FIREWORKS photometry and spectroscopic %redshifts
%from \citet{Wuyts2008PHOTZ}.
%LPZ uses templates from \citet{BC03}
%calibrated using COSMOS \citep{Koekemoer2007} photometry and
%spectroscopic redshifts
%as described in \citet{Ilbert2009}.
%Further details on these methods can be found in the %aforementioned
%references.
%While similar, the two methods serve as important cross-checks %of one
%another.

\emph{Thanks for updating this. The only comment missing is some conclusion about the final photo-z adopted (and the reason). For example, the reader needs to know where the curves presented in Fig. 9 and 11 come from (which photo-z method).}

Thank you, we have updated the figure captions to reflect that these are BPZ SED fits. Also, as we have emphasized, LePhare gives similar results.

Comment 3
%%-What are the possibilites explored in terms of reddening, ages, SFH,
%%metallcity, upper limits in the photometry, when running the phot-z
%% codes?
% We note that BPZ uses a library of empirically calibrated
% templates
% (Ben\'itez, private communication), similar to that obtained in
% Ben\'itez
% et al. 2004. Since galaxy properties are not the purpose
% of this paper,
% for the redshift estimation we use relatively small
% libraries to avoid color degeneracies. The templates span a
% large range
% of colors from elliptical to
% starbursts templates, which are representative of the galaxy
% population
% found in clusters.
% These libraries are not big enough to provide accurate
% estimates % of SFH,
% ages and metallicity, and this will be detailed in our
% upcoming methodreview papers.

\emph{My comment was not to get individual physical values for the lensed galaxies, but rather to check the range explored, the most important parameters being the reddening and the SFH. The
LPZ code uses a range of templates from BC03, with different SFH, and also allows a range of reddening values to be used, this is just to include one sentence summarizing the parameter space explored.}


The templates are empirically generated, describing well the full range of galaxy colors found in multiband catalogs such as COSMOS and FIREWORKS (less than $sim1\%$ outliers for high quality spectroscopic samples) and therefore implicitly encompass all the range of metallicities, extinctions, and star formation histories of real galaxies. Specifically, the color-redshift space explored in the template library is the same as described in the COSMOS paper (Ilbert et al. 2009). In that paper a very careful work is described on optimizing the templates to match the color-redshift relation they find in the 30 COSMOS bands and using diverse spectroscopic redshift samples. We believe that these templates are optimal for the CLASH observations as well, and will develop this in a soon-to-come paper (Jouvel et al. 2011 / in preparation).

Explicitly, the LPZ template library includes nine galaxy templates generated by Polletta et al. 2007 with the code GRASIL Silvia et al. 1998 (3 ellipticals and 6 spirals) and 12 BC03 with starbursts (SB) ages ranging from 3 to 0.03 Gyr to better reproduce the bluest galaxies. We used Calzetti et al 2000 extinction laws with values of E(B-V) = 0.1 to 0.5. We also include the impact of emission line strength in the photo-$z$ estimation, as described in Ilbert et al. (2009).

We have now made corresponding (minor) changes in the text, so that the paragraph describing the photometric redshifts now reads: ``Based on the 16-filter photometry,
we obtain photometric redshifts using BPZ \citep{Benitez2000, Benitez2004, Coe2006}
and LePhare (LPZ hereafter; \citealt{ArnoutsLPZ1999,Ilbert2006BPZ}).
These two methods yielded some of the best results of all photo-z methods tested by the PHoto-z Accuracy Testing group \citep{Hildebrandt2010PHOTZ}.
BPZ and LPZ are similar in that spectral energy distribution (SED) templates
are redshifted and fit to observed photometry.
BPZ currently uses 6 templates from PEGASE \citep{Fioc1997PEGASE},
calibrated using the FIREWORKS photometry and spectroscopic redshifts from \citet{Wuyts2008PHOTZ}.
LPZ uses templates from \citet{BC03} calibrated using COSMOS \citep{Koekemoer2007} photometry and spectroscopic redshifts
as described in \citet{Ilbert2009}. The templates are empirically generated, describing well the full range of galaxy colors found in these multiband catalogs (less than $sim1\%$ outliers for high quality spectroscopic samples), and therefore implicitly encompass all the range of metallicities, extinctions, and star formation histories of real galaxies. Further details on these methods can be found in the aforementioned references.
While similar, the two methods serve as important cross-checks of one another.''


Comment 4
%%- Quantitatively,how cluster members are defined in terms of
%%photometric redshifts ? Which range of redshifts is used ?
%In practice, we begin our lens modeling before the full dataset %is ready for useful photometric redshifts, so that cluster %members input into the mass model are only chosen as lying
% close to the red-sequence (and
%magnitude). These were then verified to distribute around the %cluster
%redshift when the full dataset was available, though we did not %use
%redshift cuts for choosing members. This is why in the text we %note that
%"Cluster member
%galaxies are identified as lying close to the cluster sequence %by the
%photometry described in \S \ref{obs}. In addition, using our %extensive
%16-band imaging and corresponding photometric redshifts, these %can be
%then verified as members lying at the cluster's redshift".

\emph{OK. I just wanted to add which color sequence has been used to
select cluster members. Since the UV filters are very important
as you mention in your answer, I imagine these filters has been
used for cluster selection.}

Comment 5
%%- I understand the model used for the mass distribution has 6
%%parameters. I
%%noted the "degree of smoothing S", the index of power-law q, the
%%direction of sheer and its amplitude, the factor Kgal. Is the sixth
%%parameter the "normalization of the model" according to the text ? In
%%any case this should be clarified: which 6 parameters are used, and if
%%one parameter misses a definition/symbol it should be added.
%%
%%- What are the values of the best fit 6 parameters for the
%% model ?

%Note that the explicit values obtained in the minimization do %not add any
%additional physical value here, since they are coupled to the %initial
%photometry, and the procedure described in our work.

\emph{I partially disagree. At least the final smoothing scale adopted
seems very important as other teams use this approach to model
lensing clusters and it would be very important to compare. Also, as I say below, this smoothing value and its associated error have an important effect on the overall "roundness" of the final mass distribution.}

OK, we still feel this has to be quoted with cautious and so we have now added to, or changed the text in the results section to:
"We have made use of the location and redshift information of the
multiple-images to fully constrain the mass model. We find that the critical curve for a source
at $z_s=2.55$ (systems 3-4) encloses..."

to -->

"We have made use of the location and redshift information of the
multiple-images to fully constrain the mass model. In our minimization procedure, we obtain for most important parameters controlling the mass distribution, values of $q=1.08\pm0.08$ and $S=12\pm2$, but note these are highly coupled to the photometry used to construct the mass model, and to our procedure detailed in \S 3.

We find that the critical curve for a source
at $z_s=2.55$ (systems 3-4) encloses..."

Comment 6

%%Fig.4: What is the smoothing scale used in this figure ? How
%%does this
%%smoothing scale
%% affect the "roundness" of the mass distribution ?
%We did not use explicitly any smoothing here. This is literally %the resulting mass distribution, in spaces of \Delta\kapaa=0.1. ...

\emph{I disagree. Implicitly, there is a smoothing scale for the "smooth" component of the mass distribution, which comes from the parameter S. Since this smoothing will circularize the mass
distribution, the resulting roundness will strongly depend on the final value (and uncertainty) of this parameter.}

Agreed, but still this is already embedded in our mass model, which is shown in this figure. There is no smoothing applied in generating the figure. We believe our response to the previous comment above now settles it.

%%- The authors cannot say something like
%%"where most clusters are expected to have larger critical area %%and
%%thus larger numbers
%%of multiple-images spread over a large redshift range, we will %%be
%%able to put statistically-significant constraints on the %%cosmological
%%parameters."
%%when we know it is likely not true.
%While we cannot know for certain at this stage what the precise %Einstein
%radius distribution for our sample is, we can infer, based on %x-ray
%scaling relation arguments, that A383 probably has one of the %smallest
%Einstein radii - it has both the lowest x-ray temperature and %x-ray
%luminosity in the CLASH sample. Furthermore, as was shown for %A1689
%(e.g., Jullo et al. 2010) - reasonable constraints can be put %on the
%cosmological parameters even using only one cluster with ~20 %multiply
%imaged background galaxies. Based on the number of multiply-
%imaged
%systems already found in the high-magnification clusters in our %CLASH
%sample, combined with the substantial number expected even in %the x-ray
%selected subset of 20 clusters in our sample, one would %anticipate a
%significant reduction in the uncertainty on the cosmological %parameters.

\emph{I don't follow this argument. In Jullo et al, the authors have access to a much larger sample of multiple images than the one finally used (at least a factor of 3 more images), they select the more isolated ones. Therefore, based on A383 having only
14 images with spectroscopic redshift, it is very unlikely that 20 images will be useful for this purpose per individual cluster. I ask the authors to remove or strongly tone done such claim. }

The idea is that one can combine multiple-images, or constraints, from all 25 clusters together, and so we should have eventually hundreds of multiple images to constrain cosmology with. To make it clearer in the text we simply changed: "With a sample of 25 CLASH clusters however, where most clusters are expected to have larger critical area and thus larger numbers of multiple-images spread over a large redshift range, we will be able to put statistically-significant constraints on the cosmological parameters"
to -->
"With a sample of 25 CLASH clusters however, where most clusters are expected to have larger critical area and thus larger numbers of multiple-images spread over a large redshift range, we will be able to put statistically-significant constraints on the cosmological parameters, combining the information from all clusters together."



We thank again the referee for these useful comments.
Best wishes,
the CLASH team.  
